"I Like Sunnie More Than I Expected!": Exploring User Expectation and Perception of an Anthropomorphic LLM-based Conversational Agent for Well-Being Support

The human-computer interaction (HCI) research community has a longstanding interest in exploring the mismatch between users' actual experiences and expectation toward new technologies, for instance, large language models (LLMs). In this study, we compared users' (N = 38) initial expectations against their post-interaction perceptions of two LLM-powered mental well-being intervention activity recommendation systems. Both systems have a built-in LLM to recommend a personalized well-being intervention activity, but one system (Sunnie) has an anthropomorphic conversational interaction design via elements such as appearance, persona, and natural conversation. Results showed that user engagement was high with both systems, and both systems exceeded users' expectations along the utility dimension, highlighting AI's potential to offer useful intervention activity recommendations. In addition, Sunnie further outperformed the non-anthropomorphic baseline system in relational warmth. These findings suggest that anthropomorphic conversational interaction design may be particularly effective in fostering warmth in mental health support contexts.

==> archive.tex <==
The field of conversational agents has been significantly advanced by the Large Language Models (LLMs), enabling more natural and context-aware interactions across various domains. LLM-powered conversation agents(CA) are capable of better understanding nuances and generating personalized responses, making it useful in domains such as healthcare, education, and customer service \cite{}. 

In particular, LLM-based CA have shown great potential in the context of mental well-being support \cite{}. These agents engage users in meaningful conversations, provide personalized suggestions, and help users to develop strategies for managing mental health challenges such as stress and anxiety, prompting positive psychological outcomes and contributing to overall happiness and well-being. However, several concerns arise regarding LLM-based CA under this context, including the accuracy of the information, the ability to understand the user's context and show empathy, the potential of privacy issues and reinforcing biases. Such limitations could potentially have adverse effects on users' mental well-being.   

It is crucial to have reliability and transparency in these agents to make sure users receive appropriate guidance and support for their mental health needs to further build and maintain user trust. One way to enhance the reliability of CA is to provide an evidence-based feature for explainability and transparency, such as citations in GPT generated responses, which could offer users the opportunity to verify the sources of information and validate the accuracy of the responses\cite{}. ChatGPT-4, for example, had added this feature in their recent release to provide transparency and explainability regarding the source of the information. However, it is not clear how this explainable AI feature could be used and its impacts on user trust and engagement in LLM-based CAs for mental well-being support.

We use Sunnie, the LLM-based CA in Flourish Science, to understand users' experiences with LLM-based CA for mental well-being support. Flourish aims to translate psychological research knowledge into engaging and interactive activities to help people find more happiness and well-being, enhancing user trust and further promoting happiness management and influencing behavior changes. We are focusing on the specific interaction in "Dive deeper with Sunnie" which allows user to engage in a more in-depth conversation with LLM-based CA about their current feelings or mental challenges where the agent provide users with actionable and personalized suggestions.   

In this work, our goal is to understand the impacts of this explainable AI feature in user engagement, trust, and potential behavioral change, and explore the potentials in facilitating human-AI trust and enhancing transparency and reliability of LLM-based CA for mental health support. 
We aim to explore and address following research questions:

\textbf{RQ1: User experience \&engagement}: What impact does the evidence-based AI explainability feature have on user engagement with LLM-based CA? 

\textbf{RQ2: User trust}: How do users perceive the quality and reliability of mental health tips provided by the agent with and without citations? How does the inclusion of citations in responses of LLM-assisted CA, influence user trust in the context of mental health management?

\textbf{RQ3: Behavioral change}: How does the citation feature affect the user's understanding and acceptance of personalized mental health tips?

\textbf{Participants}
We will recruit 30 participants to use "Dive Deeper with Sunnie" for 21 days. Participants will be adults aged 18 and above who are comfortable interacting with conversational agents and have an interest in mental well-being support. We will ensure a diverse sample in terms of age, gender, and cultural background to generalize the findings.


The study will assess their experiences at three different interaction stages: pre, during and post. 

\textbf{Pre-stage:} Participants will complete a set of questionnaires to measure their personality traits, psychological well-being, mood, and readiness to change health behavior for better well-being as a pretest. They will also attend a 1-hour focus group workshop where the research team will introduce the functionalities of Sunnie (a version without citations) and instruct participants to interact with Sunnie themselves. After the workshop, participants will complete questionnaires regarding user experience, adopting The Subjective Assessment of Speech System Interfaces (SASSI).

\textbf{During-stage: }Participants will be divided into two groups: a control group will use a version that doesn't provide citations (the same version used in the workshop), and multiple treatment groups will use versions that provide citations but vary in UI designs around how the citation is presented to account for the main confounding factor.

\textbf{Post-stage: } A validation group will cross-validate the findings from the control and treatment groups to test the robustness of the findings and ensure that the results are not specific to a version with citations. Participants will finish follow-up questionnaires and participate in semi-structured interviews. 

To answer RQ1, we will measure both user experience and user engagement, including interaction logs analysis and user experience questionnaires. For the treatment groups, we could measure Click-Through Rates (CTR) of the citations, dwell time on citation content, etc. To answer RQ2, we will design questionnaires and conduct semi-structured interviews with participants to explore human-AI trust. To answer RQ3, we will provide a self-reported questionnaire to assess the acceptance of personalized mental health tips, and possibly measure physical data during the study period, such as daily walk time, daily sleep time, daily mediation time, etc.

We expect to find that the evidence-based AI explainability feature positively impacts user engagement with LLM-based CAs for well-being support. Specifically, we anticipate that users in the treatment groups (with citations) will show higher interaction rates and greater overall satisfaction compared to the control group (without citations). We also expect that the inclusion of citations will enhance user trust in the mental health tips provided by the agent, as users can verify the sources of information. Furthermore, we hypothesize that the citation feature will improve users' understanding and acceptance of personalized mental health tips, leading to a greater likelihood of behavioral change.

The study will suggest that the integration of evidence-based AI explainability features, such as citations, can significantly enhance user engagement, trust, and understanding in LLM-based CAs for mental well-being support. This will highlight the importance of transparency and reliability in conversational agents, especially in sensitive domains like mental health.


{\color{blue}
It would be helpful if you could turn the track changes function on. I think it is disabled for the current status of your account.

Some feedback from Feb 28 writing workshop by Ruishi:

In paragraph 2, “including the accuracy of the information, the ability to understand the user's context and show empathy, the potential of privacy issues and reinforcing biases. Such limitations could potentially have adverse effects on users' mental well-being”, it seems like the project is about “accuracy of the information”. So it would be better to highlight that specifically.

In paragraph 3, “such as citations in GPT generated responses”. My concern is that presenting evidence in the form of “citation” could be difficult for CAs.

In paragraph 3, “it is not clear how this explainable AI feature could be used and its impacts on user trust and engagement in LLM-based CAs for mental well-being support.” I remembered there are works about XAI features \& trust, maybe starting from this is a better way to identify research gap.

Transition between paragraph 3 and 4. It seems a bit out of the blue to directly introduce Sunnie.
}



\section{A description of the study}

Project Objective
We aim to evaluate the effectiveness of 
{\color{blue}an} anthropomorphic LLM-based conversational agent (Group B) in supporting mental well-being compared to non-anthropomorphic conversational agent (Group A), in terms of mood change, perceived helpfulness, action taking, and general expectations of LLM-based conversational agent over a 7-day period

Pre-Study Survey:
Collect baseline data on participants' well-being, perceived helpfulness and general expectations of LLM-based conversational agents.
Daily Check-Ins:
Participants will interact with their assigned conversational agent once daily.
Before each interaction, participants will complete two questions assessing their mood and emotional keywords
After each interaction, participants will complete two {\color{blue}more} questions assessing their mood and emotional keywords. Daily completion of recommended activity will be collected via the typeforms.  
Post-Study Survey:
At the end of the 7-day period, participants will complete a final survey assessing their overall experience, mood change, perceived helpfulness, action-taking, and any changes in their expectations of LLM-based conversational agents.
(potentially) Some participants will be invited to participate in semi-structured interviews for further reflections of their experience by answering several interview questions. 

==> sections/introduction_prev.tex <==
 \section{Introduction}



Our society is facing a growing mental health crisis, with increasing demands for support and limited access to mental health professionals such as therapists and counselors \cite{who2023, apa2022impact}. 
In response, research has identified key factors contributing to well-being (e.g., the PERMA model~\cite{seligman2011}) and has designed a variety of evidence-based activities, including physical and cognitive activities, to improve well-being~\cite{walsh2011lifestyle, Penedo2005ExerciseAW}. 
However, despite the wealth of information on evidence-based strategies to improve well-being, most people still find it difficult to integrate these activities into their daily routines, even when they understand the potential benefits~\cite{Schueller2013, Prochaska1997}. 
This gap between awareness and action (i.e., the knowledge-action gap) can be attributed to several factors, including lack of motivation, perceived difficulty in adopting new behaviors, and the absence of personalized guidance~\cite{knittle2018can, Ryan2000, Prochaska1997}. 

Against this backdrop, the emergence of AI, and more specifically AI-based chatbots, presents a promising avenue for overcoming these barriers. Indeed, recent research has explored the potential of chatbots as an innovative tool to bridge this knowledge-action gap in well-being support ~\cite{stephens2019feasibility, piao2020use, kramer2020components, kramer2019investigating, kunzler2019exploring, kocielnik2018reflection, zhang2020artificial, maher2020physical, fadhil2019assistive, Oh2021ASR, Krame_2020}. 
By providing conversational and interactive support, chatbots have shown promise in promoting user engagement and encouraging the adoption of healthier behaviors \cite{Oh2021ASR, Aggarwal_Tam_Wu_Li_Qiao_2023}. 
Current research on chatbot interventions primarily focuses on lifestyle improvements--such as promoting physical activity, improving dietary habits, and enhancing sleep quality--to support well-being ~\cite{kramer2020components, Aggarwal_Tam_Wu_Li_Qiao_2023, Oh2021ASR, Singh2023SystematicRA, Perski2019DoesTA, fan2021utilization, wang2021cass}.
However, these interventions often fall short due to limitations such as inadequate understanding of context, difficulty handling complex conversations, and lack of personalization~\cite{kramer2020components, Aggarwal_Tam_Wu_Li_Qiao_2023, Oh2021ASR, Singh2023SystematicRA,perski2017conceptualising, zhang2022storybuddy}.

The emergence of large language models (LLMs) presents new possibilities to enhance well-being support through LLM-based chatbots, with their superior natural language processing capabilities fostering a more nuanced understanding of context and improved handling of complex conversations \cite{de2023benefits, torous2024generative, van2023global, yang2024talk2care, mahmood2023llm, chan2023mango}.
Such advantages of LLMs could lead to more human-like and relatable conversational experiences, potentially increasing user engagement \cite{loh2023harnessing, ma2023understanding, Song2024TheTC}.
The integration of anthropomorphic features in LLM-based agents presents a promising avenue to deliver interactions that are not only more engaging but also more effective in motivating users to take action towards well-being ~\cite{seeger2018designing, laban2021perceptions, Bowman_Cooney_Newbold_Thieme_Clark_Doherty_Cowan_2024, chinmulgund2023anthropomorphism}.
Despite the advancements in LLMs, there is limited research on their use in promoting activities for well-being support. 
Most existing studies focus on improving personalization and providing a more human-like experience through conversations, but rarely focus on facilitating action-taking or recommending activities to practice well-being \cite{Song2024TheTC, Hua2024LargeLM, ma2023understanding, loh2023harnessing, liu2023chatcounselor, yao2023development, cho2023evaluating}. 

Furthermore, despite these technological advancements, people’s expectations of AI systems may still limit their adoption. Previous research has shown that users often hold expectations that AI systems are high in agency (e.g., capacity for self-control) but low in experience (e.g., capacity to feel)~\cite{gray2007dimensions}. These expectations might limit how much users are willing to rely on AI-driven mental health support, especially given that mental health support requires more compassion and relational warmth, which may be perceived to stem from the capacity to feel. While previous research has examined expectations versus experience in other domains such as gaming ~\cite{michalco2015relation} and conversational agents in various contexts~\cite{luger2016like, cho2019once}, we build on this work by examining this within the context of well-being applications, and by specifically comparing anthropomorphic versus non-anthropomorphic AI designs.


Thus, a critical yet unaddressed question is how: 1) the design of LLM-based systems, especially the incorporation of anthropomorphic features, influences users' perceptions and their willingness to engage in actions that support well-being, and 2) whether and to what extent users underestimate the capabilities of these AI systems.

Thus, our study is guided by three research questions:
\begin{itemize}
    \item \textbf{RQ1}: How do anthropomorphic designs of LLM-based conversational agents for well-being support shape users' \textbf{perceptions} of the systems?
    \item \textbf{RQ2}: How do such designs influence users' \textbf{engagement} in adopting recommended well-being activities? 
    \item \textbf{RQ3}: To what extent do users' \textbf{expectations} of LLM-based systems align with their actual experiences of these systems?
\end{itemize}

We introduce \system, an anthropomorphic LLM-based conversational agent designed to offer personalized well-being support and recommend practical actions grounded in positive psychology and social psychology research. 
\system is an ``AI happiness coach and companion'' developed by Flourish Science, a public benefit corporation with the mission of ``personalizing the science of happiness and well-being to make it accessible, actionable, simple, and fun, thereby providing proactive and just-in-time mental health and well-being support.'' The version tested in the current study is powered by GPT-4 \cite{achiam2023gpt}, an advanced LLM, to offer more human-like interactions, thereby enhancing personalization and encouraging users to take action to improve their well-being. 


We hypothesize that incorporating anthropomorphic features into the design of \system will lead to more positive perceptions and, in turn, increase user engagement and the likelihood of adopting the recommended well-being activities. Additionally, we hypothesize that users will underestimate the capabilities of the anthropomorphic design, particularly in its ability to convey warmth.
To test our hypotheses, we conducted an empirical user study that compared users' expectations and perceptions of two designs: \system, an anthropomorphic conversational agent, and a non-anthropomorphic, non-conversational, LLM-based activity recommendation system.  

The core contributions of this paper are tri-fold:
\begin{itemize}
    \item Describe the design and development of \system, an anthropomorphic LLM-based conversational agent equipped with emotion regulation coaching and well-being activity recommendations, aimed at enhancing personalized well-being support and facilitating proactive well-being management.
    \item Report findings and insights from an empirical 3-day, within-subject user study through quantitative and qualitative analysis examining how anthropomorphic designs shape user perceptions, engagement, and how these perceptions align with their initial expectations. 
    \item Provide design considerations derived from our study results to foster the future development of LLM-based well-being support systems in terms of more personalized and effective support.
    
\end{itemize}


